Frozen Feature Augmentation for Few-Shot Image Classification

Training a linear classifier or lightweight model on top of pretrained vision model outputs, so-called 'frozen features', leads to impressive performance on a number of downstream few-shot tasks. Currently, frozen features are not modified during training. On the other hand, when networks are trained directly on images, data augmentation is a standard recipe that improves performance with no substantial overhead. In this paper, we conduct an extensive pilot study on few-shot image classification that explores applying data augmentations in the frozen feature space, dubbed 'frozen feature augmentation (FroFA)', covering twenty augmentations in total. Our study demonstrates that adopting a deceptively simple pointwise FroFA, such as brightness, can improve few-shot performance consistently across three network architectures, three large pretraining datasets, and eight transfer datasets.

==> figures/first_page.tex <==
\begin{figure}
  \centering
\includegraphics[width=\columnwidth]{figures/images/first_page.pdf}
  \caption{Few-shot results averaged across all eight test sets, including, CIFAR100 \cite{Krizhevsky2009}, ILSVRC-2012 \cite{Deng2009, Russakovsky2015}, and SUN397 \cite{Xiao2010,Xiao2016}. We use cached features from an L/16 model \cite{Dosovitskiy2021} pretrained on JFT-3B \cite{Zhai2022}. Our method, \ie, a multi-head attention pooling (MAP) \cite{Lee2019f} head trained on frozen feature augmentation (FroFA), shows superior performance across shots. Further, MAP + FroFA, 5-shot, even equals MAP, 10-shot (dashed black line).}
  \label{fig:first_page}
\end{figure}

==> figures/i21k_results.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{figures/images/i21k_all_models_wd.pdf}
\caption{\textbf{Top-1 accuracy of our best FroFA for ImageNet-21k models} on \textit{our} ILSVRC-2012 test set trained on few-shot subsets of the ILSVRC-2012 training set. Absolute gains to the MAP and linear probe baseline are reported. We sweep across a base sweep (\cf \cref{sec:training_details}) and a brightness level sweep (\cref{sec:appendix_augmentation}) to first find the best setting on \textit{our} ILSVRC-2012 validation set for each model.}  \label{fig:i21k_all}
\end{figure*}

==> figures/image_feature_pair.tex <==
\begin{figure}
  \centering
\includegraphics[trim={0 0.7cm 0 0},clip,width=\columnwidth]{figures/images/image_and_features.pdf}
  \caption{\textbf{An image-features pair}. We take an ILSVRC-2012 \cite{Russakovsky2015} image of shape $224\!\times\!224\!\times\!3$ and an L/16 vision transformer \cite{Dosovitskiy2021, Zhai2022} pretrained on JFT-3B \cite{Zhai2022} to extract (reshaped) features $\boldsymbol{f}'$ of shape $14\!\times\!14\!\times\!1024$ (output of last Transformer block). We depict the first six feature channels $\boldsymbol{f}'_c$ of shape $14\!\times\!14$. The color gradient indicates the exact value. Note that feature channel $\boldsymbol{f}'_{c=6}$ (highlighted in \textcolor{red}{red}) shows a structural resemblance with the input.}
  \label{fig:image-feature-pair}
\end{figure}


==> figures/jft3b_results.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{figures/images/jft3b_all_models_wd.pdf}
\caption{\textbf{Top-1 accuracy of brightness c$^2$FroFA for additional JFT-3B models} on \textit{our} ILSVRC-2012 test set trained on few-shot subsets of the ILSVRC-2012 training set. Absolute gains to the MAP and linear probe baseline are reported. We sweep across a base sweep (\cf \cref{sec:training_details}) and a brightness level sweep (\cref{sec:appendix_augmentation}) to first find the best setting on \textit{our} ILSVRC-2012 validation set for each model.}  \label{fig:jft3b_all}
\end{figure*}
